The Role of the Internet of Things in Network Resilience

Disasters lead to devastating structural damage not only to buildings and transport infrastructure, but also to other critical infrastructure, such as the power grid and communication backbones. Following such an event, the availability of minimal communication services is however crucial to allow efficient and coordinated disaster response, to enable timely public information, or to provide individuals in need with a default mechanism to post emergency messages. The Internet of Things consists in the massive deployment of heterogeneous devices, most of which battery-powered, and interconnected via wireless network interfaces. Typical IoT communication architectures enables such IoT devices to not only connect to the communication backbone (i.e. the Internet) using an infrastructure-based wireless network paradigm, but also to communicate with one another autonomously, without the help of any infrastructure, using a spontaneous wireless network paradigm. In this paper, we argue that the vast deployment of IoT-enabled devices could bring benefits in terms of data network resilience in face of disaster. Leveraging their spontaneous wireless networking capabilities, IoT devices could enable minimal communication services (e.g. emergency micro-message delivery) while the conventional communication infrastructure is out of service. We identify the main challenges that must be addressed in order to realize this potential in practice. These challenges concern various technical aspects, including physical connectivity requirements, network protocol stack enhancements, data traffic prioritization schemes, as well as social and political aspects.

==> abstract.tex <==
%%% SECTION %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section*{}
\begin{bf}
Abstract -- TODO
\end{bf}


==> notes.tex <==
%%% SECTION %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Network Topology Evolution}
\label{sec:net}

\section{Opportunities_new}

Say: \\
++	1. The internet evolved from workstations to mobile devices, rapid deployment of those, millions of devices
++ 	2. We are on the verge to everything connecting: the internet of things (IoT): billions of devices, EU \cite{vermesan2011} Industry \cite{ericcson2011}
++ 3. explain basics of the IoT, what is it that makes it so important and different
 -- massive deployment
 -- from high performance to class 0 devices
 -- mobile, battery driven
 -- lose coupling, mesh networking
 -- diversity
 
 -- EVERYTHING IS CONNECTED - we expect IoT devices bper se to be able to speak with another
++ 4a. Show that the IoT is not as vulnerable to disasters
++	4. Give examples
 -- Typical bandwidth: \cite{onwuka2013}
 
++ 5. Map to communication needs from section \ref{sec:commdis} (2)

++	6. Show further opportunity: Sensor networks can be utilized to bring additional situational data: temperature in fire scenarios, radiation measurement (Fukushima), air quality in bio/chemical attacks

6. Plot opportunity scenarios:
 -- Text-based emergency broadcasts
 -- 911-alike emergency calls, e.g. buried persons can call/text for help
 -- text/voice communication between first responder teams

\section{Challenges}
---Challenges---

0. How to accomplish connectivity
 -- needs to be configuration less
 -- spontaneous
 -- multi-hop
 -- scalable (both for radio medium and routing)

1. HW
 -- different radio frequencies, routers needed, multi-radio devices
 -- reliability, dependencies on signal strength
 -- medium jamming (interference between frequencies bands, to much use of used bands)
 
2. SW:
 -- we expect up to the network layer that devices are able to talk to each other
 -- this is still not enough
 -- scalable and robust routing protocols that all devices understand
 -- applications are missing (emergency mode as in 911 calls)
 -- Prioritization of services/traffic: how to prevent people from using all the bandwidth using youtube when emergency services are required
 
3. Security:
 -- if something like emergency mode would exist, how to prevent anyone to enable it
 -- secure operational data from police/fire-fighters against eaves-dropping, terrorists
 
 
 \newpage
\subsection{Hardware}
A Hardware connectivity
- different radio standards: 3G, Wifi, 802.15.4, bluetooth, nfc, all on different frequencies, different modulation
- modern devices with multiple radios are designated for routing over hw-gaps
- frequency jamming, small radio bands for communication

A1 Hardware limitations
- Sensor nodes are optimized for a long battery lifetime
- It needs to be investigated how they would behave in scenarios where they are constantly routing network traffic. Are the battery lifetimes still sufficient?
- Especially boarder routers are often connected to the power grid, which is vulnerable in disaster scenarios. How can they be compensated with other technologies, or do we need battery packs on them?

Hardware: Standardization efforts towards unified radio technologies are already fairly progressed. IEEE802.11 is an worldwide industry standard and heavily used and deployed. IEEE804.15.4 is ratified an increasingly adapted by the industry and consumer products. Multi-radio devices are further becoming commonly spread, as modern cell-phones provide at least WiFi, Bluetooth and NFC, so bridge or router capabilities are given by the hardware.

[Add bluetooth:  IEEE 802.15.1]
[No cellphone with 802.15.4 capabilities]

\subsection{Software 1}





\subsection{Prioritization}
D Prioritization of traffic
- very limited bandwidth and throughput, so most important traffic needs to be routed
- what about sensors primary functionality of sending sensor data, this could lead to unwanted traffic
- solution could be to put devices into emergency mode: just route selected traffic and do routing, but do not emit data on their own, now updates, no pull/push services
\newpage
\section{ONE}

Matthias:
[What data needs to be transmitted: base information, people, orginizations]
[Look for reports: what kind of communication is needed]
[see: Fukushima, Katrina]
[Work out, that this data is generally able to be transmitted by IoT]
[Parties: NGOs]
[Haiti: The main internet backbone survived, leaving the last mile out of order [Computerworld]]
[Connectivity vs Service]
[IoT: IPv6 enabled devices]

Manu:
[Start discussion on what services are important and needed]
[Compare: Emergency mode in Cell-phones: call 911 anytime]
[Equivalent to this in spontaneous networks]
[Example: Ping from people in danger]
[Gap: not only time. also man power, material]
[Limited connectivity: also could be used to continue reading sensors: fukushima etc]




%-- subsction ---------------------------------------------------------------------------
\subsection{Today’s Communication Topology}
Todays communication networks topology on two views: HW (topology) and SW (arch)

HW: onion-like architecture with fast and reliable backbone in the center and shells with decreasing bandwidth and reliability around

SW: Standardized, layered internet protocol stack including highly scalable and agreed on routing protocols, platforms and middle-wares

%-- subsction ---------------------------------------------------------------------------
\subsection{Internet of Things}
Definition: TODO: good one with source needed

Collection of loose coupled, wireless devices, usually in a mesh-like configuration, possibly (partly) mobile and dense

Typical (HW) parameters: wireless, radios on ism bands (sub-GHz, 2.4GHz), bandwidth ca 10 to 2000kbits, ca 100m range

Typical (SW) parameters: as of today no industry wide standards for protocols (though first ambitions as in 6lowpan)

%-- subsction ---------------------------------------------------------------------------
\subsection{Topology Change towards IoT}
Very fast growing number of IoT-enabled devices and therefore fast growing density especially in urban areas \cite{vermesan2011}

Prevalent mix of conventional star- and mesh-topologies on the outer shells of the "internet onion"



In the foreseeable future there will be a massive increase of deployed IoT-enabled devices around the world \cite{vermesan2011}. The main characteristics of these devices are that they are communicate wireless and are battery driven. These attributes make them largely resistant against the in section \ref{sec:disasterrequirements} described fault modes. Even if large parts of the conventional infrastructure is destroyed, the chances are quite good that there will still be a significant number of working IoT-enabled devices in the disaster area.

Assumed the above mentioned assumption will occur, it would be optimal to use the communication capability for the most important services as listed in section \ref{sec:disasterrequirements}. Even when assuming that the usable throughput will only be a fraction of the pre-disaster available capability, it could be utilized by first-responders to increase their coordination. 




For providing useful communication services, IoT-enabled devices have to connect spontaneously to large networks covering areas that are affected by a disaster. In optimal cases these networks have not only to provide end-to-end connectivity inside these areas but are also capable of providing connectivity to the rest of the internet. These section will list the requirements on the single nodes and the network architecture to be able to do so.

For a connectivity covering large areas, different classes of devices need to agree on a set of attributes that empower them to connect to each other. These attributes can be roughly split in two groups: they have to be physically able to speak to one-another and they have to use the same semantics. 

The first class of attributes can be broken down to radio-standards, modulation techniques, device locations and signal strength. These can all be grouped to hardware requirements.

The second class of attributes contains all means of semantic properties. Generally these are include the network stack, the applications running on top of it and the data formats that are exchanged. All of these attributes are part of the software and can hereby grouped into requirements for the software.







[Recovery: temporal networks/base stations for complete recovery or for 

Manu:
[GAP: configuration less connectivity: huge improvement of today's situation]



%%% SECTION %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{In Case of Disasters}


%-- subsction ---------------------------------------------------------------------------
\subsection{Impacts}
Depend on nature of disaster, but common impacts: 
\begin{itemize}
\item large number of people affected
\item more or less large areas of destruction 
\item limited or none access to supply, accommodation and communication
\item especially for communications: loss of power grid and backbone and inter-node connectivity
\end{itemize}


Common: break down and overload of communication infrastructure

Common: need for communication: HFNs, BOS, people

Phases: during, after disaster

%-- subsction ---------------------------------------------------------------------------
\subsection{Hastily Networks}

First Responders: Hastily networks - definition and more in \cite{denning2006}, dependent on communication networks

Further needed communication services: phone service for affected people, news, social networks, logistics services


%-- subsction ---------------------------------------------------------------------------
\subsection{Technical Requirements}
First priority is the communication for authorities and organization responsible for safety (german: BOS)

Restoration of void and data communication: Mobile (GSM, 3G), Internet, phone

Existing work on how to temporary restore these capabilities with satellite up-links, mobile base stations etc.

But question of interest: can the combination of a dense distribution of IoT-enabled devices and spontaneous mesh networks (partly) enable these services without installation/configuration instantly in disaster scenarios?



%-- subsction ---------------------------------------------------------------------------
\subsection{Fault Modes for Communication Infrastructure}
What are the typical effects of large-scale disasters on the in section \ref{sec:net} described communication networks

Traffic: decreased (streaming, multimedia) vs. increased (communication, social networks)

Permanent: broken wires, physical damaged routers, collapsed buildings or towers

Recoverable: power outage, overload conditions,




%%% SECTION %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Disaster Resilience through Technology}

%-- subsction ---------------------------------------------------------------------------
\subsection{Applications}
End-to-end communication for different integrity levels: response forces, between relatives, social communication, news
Broadcasts: safety warnings (flood, weather, chemicals)

Different radio standards: a lot of proprietary work, standardization attempts with IEEE802.15.4

Different SW stacks: today dominated by proprietary protocols, first standardization efforts via 6lowpan

%-- subsction ---------------------------------------------------------------------------
\subsection{Interoperability}

IoT enabled devices, Spontaneous wireless networks

Hardware: Radio standards, gateways

Software: Network stack and user protocols

Network stack: today dominated by proprietary protocols, first standardization efforts via 6lowpan


%-- subsction ---------------------------------------------------------------------------
\subsection{Disaster Mode?}
Possible solution is a common "disaster mode", in which all IoT devices can be switched to for providing services for hastily network participants

This would raise severe security questions



%%% SECTION %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Conclusions}
Network infrastructure is changing towards self-contained (mesh) cells

Hardware and topology could be exploited for post disaster utilization

Software does not allow this utilization so far, a lot of work to be done

Thousands of small, battery driven, wireless nodes are resilient against most disaster infused fault modes







\newpage \newpage
\section{Literature}
These I intend to base the article on:

Spontaneous (hastily) networks in disaster scenarios:
\begin{itemize}
\item \cite{onwuka2013}
\item \cite{denning2006}
\item \cite{tornqvist2009}
\item \cite{nelson2011}
\end{itemize}

About the future development of IoT
\begin{itemize}
\item \cite{vermesan2011}
\item \cite{mattern2010}
\item \cite{sundmaeker2010}
\end{itemize}

General Network architecture:
\begin{itemize}
\item \cite{raniwala2005}
\item \cite{rahman2010}
\end{itemize}

Fault Modes:
\begin{itemize}
\item \cite{krings2006}
\item \cite{cucurull2010}
\end{itemize}

\section{Missing Literature}

Literature that could be interesting, but which I could not get my hands on:
\begin{itemize}
\item Mase: \cite{mase2011}
\item Oberg: \cite{oberg2011}
\item Räty: \cite{raety2010} (maybe not quite so interesting for this article, but could be interesting for SAFEST)
\end{itemize}

==> questions.tex <==
\section{Open Questions}
\begin{itemize}

\item What about differences between third/first-world? IoT deployment will differ quite significantly and the distribution of disasters tends to be at expense of poorer third-world countries (due to geographic reasons).
\item Turn-down: could massive IoT deployment increase data traffic in a way that remaining communication capabilities will fail because of overload conditions?
\item Security?!
\end{itemize}

==> titlepage.tex <==
\twocolumn[
\begin{@twocolumnfalse}
    \begin{center}
        {
        \huge
        The Impact of IoT-Enabled Devices on\\ Disaster Resilience of Communication Networks\\[0.8cm]
        }
        \begin{tabular}{ccccc}
            \textsuperscript{1}Hauke Petersen 	& 
            \textsuperscript{1,2}Emmanuel Baccelli & 
            \textsuperscript{1}Matthias W\"ahlisch &
            \textsuperscript{3}Thomas C. Schmidt &
            \textsuperscript{1}Jochen H. Schiller \\
        \end{tabular}
        \vspace*{2mm}\\
		\textsuperscript{1}Freie Universit\"at Berlin, Institut f\"ur Informatik, Takustr. 9, 14195 Berlin, Germany\\
        \vspace{2mm}
        \textsuperscript{2}INRIA Saclay \^Ile-de-France, 91120 Palaiseau (CEDEX), France \\
        \vspace{2mm}
        \textsuperscript{2}HAW Hamburg, Dept. Informatik, Berliner Tor 7, 20099 Hamburg, Germany \\
        \vspace{2mm}
        \texttt{\{hauke.petersen,m.waehlisch,jochen.schiller\}@fu-berlin.de} \\
        \texttt{emmanuel.baccelli@inria.fr, t.schmidt@ieee.org}
    \end{center}
    \vspace{5 mm}
\end{@twocolumnfalse}
]

